Systematically Assessing the Security Risks of AI/ML-enabled Connected Healthcare Systems

The adoption of machine-learning-enabled systems in the healthcare domain is on the rise. While the use of ML in healthcare has several benefits, it also expands the threat surface of medical systems. We show that the use of ML in medical systems, particularly connected systems that involve interfacing the ML engine with multiple peripheral devices, has security risks that might cause life-threatening damage to a patient's health in case of adversarial interventions. These new risks arise due to security vulnerabilities in the peripheral devices and communication channels. We present a case study where we demonstrate an attack on an ML-enabled blood glucose monitoring system by introducing adversarial data points during inference. We show that an adversary can achieve this by exploiting a known vulnerability in the Bluetooth communication channel connecting the glucose meter with the ML-enabled app. We further show that state-of-the-art risk assessment techniques are not adequate for identifying and assessing these new risks. Our study highlights the need for novel risk analysis methods for analyzing the security of AI-enabled connected health devices.

==> sections/framework.tex <==
\section{Proposed Risk Assessment Framework}\label{sec:framework}
% \url{https://docs.google.com/document/d/1NeDscS_zt-O1ewQin5eSwsS5Th0ggWWG/edit?usp=sharing&ouid=102465864342600939906&rtpof=true&sd=true}

\par Building upon the knowledge gathered from our investigation into existing risk assessment methodologies, this section outlines the relevant factors essential for a more comprehensive analysis of the risks inherent in AI/ML-enabled medical devices. Our examination has revealed deficiencies in the current risk assessment methodologies. Most notably, they frequently neglect the factor of \textit{detectability} and overlook another one that we call \textit{ease of mitigation} which pertains to the availability of any remediation methods and the determination of responsibility for carrying them out. Additionally, we propose revisions to the descriptions of common factors, with an emphasis on their impact on the AI/ML model as a whole, rather than individual components.
%\par We do this, considering their connectivity with peripheral devices, and introduce new factors that were previously not taken into consideration.


As previously noted, delivering a comprehensive end-to-end risk analysis is crucial due to the interconnected nature of these systems. If a vulnerability is exploited in peripheral devices or communication channels, it allows an adversary to read or modify the data being transmitted, or even initiate a Denial of Service (DoS) attack. These vulnerabilities have the potential to spread throughout the entire system, ultimately affecting the performance of the ML model and resulting in inaccurate predictions. For instance, adversaries may corrupt data by introducing perturbations to the inputs ~\cite{chen2020ecgadv, lal2021adversarial}, manipulate the training data ~\cite{menon2021covid}, gain access to the input/output data to construct a shadow model ~\cite{salem2018ml}, or exploit similar weaknesses, as evidenced in previous studies investigated in Table \ref{tab:knownmlattacks}. In this context, it becomes vital to pinpoint the factors that most accurately characterize the risks inherent in these systems. An optimal set of factors is anticipated to encompass all dimensions of vulnerability exposure in peripheral devices including its effects on the system, the ease of exploitation by attackers, the scale of user impact, and the ease of detection and mitigation. Therefore, an ideal risk analysis should consider the following factors: \textit{(1) Damage Potential, (2) Exploitability, (3) Affected User, (4) Detectability, (5) Ease of Mitigation}.
\par To the best of our knowledge, many studies in the current body of literature \cite{mahler2020new,yaqoob2019integrated,ngamboe2021risk, mahler2022cyber} have overlooked the factor of \textit{\lq Detectability\rq} since they have typically defined the risk solely as the product of severity and occurrence. Moreover, none of the existing research has integrated the concept of \textit{\lq Ease of Mitigation\rq} into their risk analysis. Therefore, in our study, we not only introduce a new factor to the risk analysis process but also offer an adjusted description of how the common factors should assess associated risks.
\par \noindent \textbf{Detectability:} As explored in the preceding section, it has been established that STRIDE, CVSS, and some other studies in the literature \cite{mahler2020new,yaqoob2019integrated,ngamboe2021risk, mahler2022cyber} do not take the factor of detectability into account. The lack of this factor results in an unrealistic assessment of vulnerability risks, as vulnerabilities that are easier to detect tend to have lower potential impacts on the system, ultimately minimizing the overall harm to users. Considering our investigated BGMS, the risk associated with the detectability factor in the case of an attack on Bluetooth communication at the point when data is received by the mobile application would be lower compared to the situation when the data is manipulated while being sent to the ML-engine, since the abnormal patterns in the blood glucose level can be easily seen and flagged by the mobile application. 
%Such detection would enable the prevention of erroneous data insertion into the ML engine, consequently averting inaccurate insulin dosage predictions.
\par \noindent \textbf{Ease of Mitigation:} Our review of existing literature revealed a notable omission, which we introduce as the \textit{`Ease of Mitigation'} factor, further categorized into two sub-factors: the responsible entity and the level of remediation. While the CVSS accounts for the remediation factor, the consideration of the responsible entity as a distinct factor in the risk analysis is a unique aspect of our proposed model. The absence of this factor will not only impact the overall risk level but will also lead to increased response times, consequently resulting in irreparable harm to the patients. The significance of this factor becomes evident when a vulnerability is exploited, as the response team needs to consider various aspects. This includes identifying the entity capable of providing a faster mitigation, evaluating scenarios where mitigation is economically advantageous, how much effort is required for mitigation and, perhaps most crucially, determining situations where mitigating minimizes the potential harm to patients. In the event of a vulnerability being exposed, the responsible entity can fall into one of four categories: Security Researcher, Third-party Vendor, Technology Vendor, or System Administrator. When the responsibility for addressing a vulnerability rests with a system administrator, the associated risk is considerably lower compared to when it lies with a security researcher. This is due to the fact that security researchers lack direct access to the system, its design, and other critical components, resulting in a longer response time. Furthermore, the level of remediation can be classified into the following categories: Unavailable, Workaround, Temporary Fix, and Official Fix. Naturally, mitigating a vulnerability becomes simpler if an official fix is already accessible, in contrast to scenarios where a new type of vulnerability arises without any available remediation, thereby significantly elevating the associated risk.

%The remaining three factors of an ideal risk analysis model comprise \textit{Damage Potential}, \textit{Exploitability}, and \textit{Affected Users}.

\par \noindent \textbf{Damage Potential:} In contrast to the considerations in DREAD or FMEA, we propose breaking down the potential damage affecting AI/ML-enabled systems into three distinct sub-factors: Confidentiality, Integrity, and Availability. This distinction is crucial, as oversimplified impact modeling may not offer a comprehensive depiction of damage severity. As an illustration, within our BGMS, the compromise of integrity could lead to irreparable health consequences for the patient, a result more severe compared to the compromise of confidentiality. Such insights would remain obscured without the inclusion of the considered sub-factors within the damage potential factor. However, regarding these sub-factors, it should be noted that we are not concerned about the loss of patients’ data from the database or the software. Those things are already taken care of by existing risk assessment techniques and are outside the scope of this work. Instead, we see the loss of confidentiality and integrity as the leakage or any modifications of feature values or model parameters respectively, and the loss of availability as the model being unable to perform normally or provide any outputs, each of these could result in wrong diagnosis and treatment, and at the worst case, fatal consequences as pointed out in Table \ref{tab:knownmlattacks}. To provide further clarification with an example, in the event that an adversary successfully compromises a portion of the input and output data, they have the potential to construct a shadow model. This situation arises if they have the capacity to monitor input and output data over an extended period, being considered as a loss of confidentiality. If the adversary can manipulate data values over a significant duration, this could contaminate the training data or directly affect the output of the model, representing an integrity compromise. Conversely, if the adversary lacks sufficient time, they may attempt to launch a DoS attack when a patient is in a critical condition, ultimately causing a loss of system availability.

\par \noindent \textbf{Exploitability:} Much like the approach suggested by CVSS, the Exploitability factor is suggested to be segmented into six distinct sub-factors: Attack Vector, Attack Complexity, Privileges Required, User Interaction, Scope, and Exploit Maturity. The Attack Vector serves to clarify how the attacker can gain access to the system. For instance, consider a situation where physical access is necessary for the attacker, either by being in close proximity to the system or having a direct physical entry. This might result in a comparatively lower risk than a scenario where the attacker can remotely initiate the attack through a network. Attack complexity and privileges required, as the terms imply, assess the difficulty involved in launching an attack and whether any specific permissions were needed, respectively. To determine whether a successful attack necessitates user engagement, the user interaction sub-factor is introduced. Furthermore, to gauge the potential impact of an exploited vulnerability on interconnected systems, the scope sub-factor is essential; altering the scope entails the vulnerability's capacity to influence not just the examined system, but also other systems interconnected with this AI-ML-enabled platform. This expansion can lead to an escalation of the cumulative risk. Finally, the exploit code maturity sub-factor within exploitability assesses the availability of functional exploit code. Higher risk is associated with the presence of such code, whereas minimal risk is attributed to cases where no exploit code is available, referred to as ``unproven''. 
\par \noindent \textbf{Affected Users:} The concluding element within our proposed framework is the Affected User factor, designed to approximate the number of users impacted in the event of a vulnerability exposure. This factor operates on the principle that an increased number of affected users correlates with higher associated risk.

%With the essential risk analysis factors in hand for assessing AI/ML-enabled medical devices, {\color{red} and to ensure consistency, a set of comprehensive descriptions for each factor is required}. 
\par In the previous section, we highlighted that the descriptions provided for the factors shared between our model, CVSS and DREAD are general in nature and may not be directly applicable in the healthcare context. This is a result of the varying risk levels associated with different domains, exemplified by the different risk levels when it comes to the loss of confidentiality in healthcare compared to web applications, as discussed earlier. Therefore, in this section, we clarified these factors and their intended use specific to the concept of AI/ML-enabled medical devices, especailly when it comes to assessing the damage potential. Table \ref{tab:factors} summarizes the considered factors in our proposed model and their intended use.  Moreover, it is worth noting that when a vulnerability is exploited, the initial analysis should give priority to evaluating the extent of damage and the method used to exploit the vulnerability. Hence, it is advisable for any analysis to adhere to this sequence before considering other factors - Affected Users, Detectability, and Ease of Mitigation - in subsequent steps. 
% \nawawy{Didn't get this. Did you mean that these should appear first and in this specific order whenever we do risk analysis? Why does order matter though since we are doing all anyway? Also, if order really matters can we reorder the factors in the way they appear in text, Table 4, and everywhere else we mention them like the case study?}
\par It is also important to note that we have chosen not to assign ratings and their accompanying descriptions to varying risk levels. This decision is rooted from the fact that risk levels can diverge significantly across distinct case studies, and different analysis teams may hold varying viewpoints. This divergence in perspectives increases the subjectivity associated with these ratings. Therefore, we acknowledge the potential for future exploration in this area.

% \mohammadreza{Yes, I changed some phrases for further clarification. In summary, we say that the very first thing you shoud analyze is the extend of damage and how the vulnerability is exploited, so the analysis shoud start with these to factors. We change the order as we wanned to bold the missing factor "Detectability" and the new one we proposed "Ease of Mitigation", first and then discuss the common factors.}


\begin{table*}[t]
\centering
\begin{tabular}{|c|M{14cm}|}
\hline
\textbf{Factor} & \multicolumn{1}{c|}{\textbf{Intended Use}} \\ \hline
Damage Potential       & To assess the level of damage in case of confidentiality, integrity, and availability. \\ \hline
Exploitability        & To address how the vulnerability was exploited with several sub-factors on the attack's vector and complexity, the required privileges, the need for user interaction, the change of scope, and the availability of exploit code. \\ \hline
Affected Users        & To assess how the number of affected users by the exploited vulnerability will pose different levels of risk.
 \\ \hline
 Detectability        & To assess how the associated risk of an exploited vulnerability will be different based on how easily it will be detected.
 \\ \hline
 Ease of Mitigation        & To address if there's an available solution and who would be responsible for mitigation in case of a vulnerability being exploited.
 \\ \hline
\end{tabular}
\caption{The proposed factors for risk analysis of AI/ML-enabled connected healthcare systems}
\label{tab:factors}
\end{table*}

% \par Building upon the knowledge gathered from our investigation into existing risk assessment methodologies, this section outlines the relevant factors essential for a more comprehensive analysis of the risks inherent in AI/ML-enabled medical devices. We consider their connectivity with peripheral devices, and introduce new factors that were previously not taken into consideration.
% % \begin{itemize}
% %     \item Desciption of the risk assessment framework, along with the rationale behind choosing the factors and the rating system for each factor - \textbf{Bold} the factors that are novel!
% %     \item Refer to the previous section and mention how the proposed framework incorporates the factors that were missing in the individual assessment frameworks
% % \end{itemize}

% % \par As previously noted, delivering a comprehensive end-to-end risk analysis is crucial due to the interconnected nature of these systems. If a vulnerability is exploited in any part of these systems, it can potentially propagate through the entire setup, ultimately impacting the ML-engine and leading to inaccurate predictions. In this context, it becomes vital to pinpoint the factors that most accurately characterize the risks inherent in these systems. An optimal set of factors is anticipated to encompass all dimensions of vulnerability exposure including its effects on the system, the ease of exploitation by attackers, the scale of user impact, and the ease of detection and mitigation. Therefore, an ideal risk analysis should consider the following factors:
% % \begin{itemize}
% %     \item \textit{Damage Potential}
% %     \item \textit{Exploitability}
% %     \item \textit{Affected User}
% %     \item \textit{Detectability}
% %     \item \textit{Ease of Mitigation}
% % \end{itemize}

% {\color{blue} As previously noted, delivering a comprehensive end-to-end risk analysis is crucial due to the interconnected nature of these systems. If a vulnerability is exploited in peripheral devices or communication channels, it allows an adversary to read or modify the data being transmitted, or even initiate a Denial of Service (DoS) attack. These vulnerabilities have the potential to spread throughout the entire system, ultimately affecting the performance of the ML model and resulting in inaccurate predictions. For instance, adversaries may corrupt data by introducing perturbations to the inputs ~\cite{chen2020ecgadv, lal2021adversarial}, manipulate the training data ~\cite{menon2021covid}, gain access to the input/output data to construct a shadow model ~\cite{salem2018ml}, or exploit similar weaknesses, as evidenced in previous studies investigated in Table \ref{tab:knownmlattacks}. In this context, it becomes vital to pinpoint the factors that most accurately characterize the risks inherent in these systems. An optimal set of factors is anticipated to encompass all dimensions of vulnerability exposure including its effects on the system, the ease of exploitation by attackers, the scale of user impact, and the ease of detection and mitigation. Therefore, an ideal risk analysis should consider the following factors: \textit{(1) Damage Potential, (2) Exploitability, (3) Affected User, (4) Detectability, (5) Ease of Mitigation}.}
% \par To the best of our knowledge, many studies in the current body of literature \cite{mahler2020new,yaqoob2019integrated,ngamboe2021risk, mahler2022cyber} have overlooked the factor of \textit{'Detectability'} since they have typically defined the risk solely as the product of severity and occurrence. Furthermore, no other research has incorporated the concept of \textit{'Ease of Mitigation'} into their risk analysis, making it a distinct and novel aspect of our proposed model. 
% \par As explored in the preceding section, it has been established that STRIDE, CVSS, and some other studies in the literature \cite{mahler2020new,yaqoob2019integrated,ngamboe2021risk, mahler2022cyber} do not take the factor of detectability into account. This omission results in an unrealistic assessment of vulnerability risks. Lack of this factor results in an unrealistic assessment of vulnerability risks, as vulnerabilities that are easier to detect tend to have lower potential impacts on the system, ultimately minimizing the overall harm to users. For the sake of simplicity, in our framework, we assign three levels of risk to the detectability factor: Low, Medium, and High. This means that the simpler the process of detecting a vulnerability, the lower the corresponding risk will be. Considering our investigated BGMS, the risk associated with the detectability factor in the case of an attack on the Bluetooth communication at the point when data is received by the mobile application would be categorized as low since the abnormal patterns in the blood glucose level can be easily flagged by the mobile application. Such detection would enable the prevention of erroneous data insertion into the ML-engine, consequently averting inaccurate insulin dosage predictions.
% \par Our review of existing literature revealed a notable omission, which we introduce as the \textit{'Ease of Mitigation'} factor, further categorized into two sub-factors: the responsible entity and the level of remediation. While the CVSS accounts for the remediation factor, the consideration of the responsible entity as a distinct factor in the risk analysis is a unique aspect of our proposed model. The absence of this factor will not only impact the overall risk level but will also lead to increased response times, consequently resulting in irreparable harm to the patients. In the event of a vulnerability being exposed, the responsible entity can fall into one of four categories: Security Researcher, Third-party Vendor, Technology Vendor, or System Administrator. When the responsibility for addressing a vulnerability rests with a system administrator, the associated risk is considerably lower compared to when it lies with a security researcher. This is due to the fact that security researchers lack direct access to the system, its design, and other critical components, resulting in a longer response time. Furthermore, the level of remediation can be classified into the following categories: Unavailable, Workaround, Temporary Fix, and Official Fix. Naturally, mitigating a vulnerability becomes simpler if an official fix is already accessible, in contrast to scenarios where a new type of vulnerability arises without any available remediation, thereby significantly elevating the associated risk.
% % \par The remaining three factors of an ideal risk analysis model comprise \textit{Damage Potential}, \textit{Exploitability}, and \textit{Affected Users}. In contrast to the considerations in DREAD or FMEA, our risk analysis approach breaks down the potential damage affecting AI/ML-enabled systems into three distinct sub-factors: Confidentiality, Integrity, and Availability. This distinction is crucial, as oversimplified impact modeling may not offer a comprehensive depiction of damage severity. As an illustration, within our BGMS, the compromise of integrity could lead to irreparable health consequences for the patient, a result more severe compared to the compromise of confidentiality. Such insights would remain obscured without the inclusion of the considered sub-factors within the damage potential factor.

% {\color{blue} \par The remaining three factors of an ideal risk analysis model comprise \textit{Damage Potential}, \textit{Exploitability}, and \textit{Affected Users}. In contrast to the considerations in DREAD or FMEA, our risk analysis approach breaks down the potential damage affecting AI/ML-enabled systems into three distinct sub-factors: Confidentiality, Integrity, and Availability. This distinction is crucial, as oversimplified impact modeling may not offer a comprehensive depiction of damage severity. As an illustration, within our BGMS, the compromise of integrity could lead to irreparable health consequences for the patient, a result more severe compared to the compromise of confidentiality. Such insights would remain obscured without the inclusion of the considered sub-factors within the damage potential factor. However, regarding these sub-factors, it should be noted that we are not concerned about loss of patients’ data from the database or the software. Those things are already taken care of by existing risk assessment techniques and are outside the scope of this work. Instead, we see the loss of confidentiality and integrity as the leakage or any modifications of feature values or model parameters respectively, and the loss of availability as the model being unable to perform normally or provide any outputs, each of these could result in wrong diagnosis and treatment, and at the worst case, fatal consequences as pointed out in Table \ref{tab:knownmlattacks}. To provide further clarification with an example, in the event that an adversary successfully compromises a portion of the input and output data, they have the potential to construct a shadow model. This situation arises if they have the capacity to monitor input and output data over an extended period, being consider as the loss of confidentiality. If the adversary can manipulate data values over a significant duration, this could contaminate the training data or directly affect the output of the model, representing an integrity compromise. Conversely, if the adversary lacks sufficient time, they may attempt to launch a DoS attack when a patient is in a critical condition, ultimately causing a loss of system availability.}

% \par Much like the approach suggested by CVSS, the Exploitability factor is segmented into six distinct sub-factors: Attack Vector, Attack Complexity, Privileges Required, User Interaction, Scope, and Exploit Maturity. The Attack Vector serves to clarify how the attacker can gain access to the system. For instance, consider a situation where physical access is necessary for the attacker, either by being in close proximity to the system or having direct physical entry. This might result in a comparatively lower risk than a scenario where the attacker can remotely initiate the attack through a network. Attack complexity and privileges required, as the terms imply, assess the difficulty involved in launching an attack and whether any specific permissions were needed, respectively. To determine whether a successful attack necessitates user engagement, the user interaction sub-factor is introduced. Furthermore, to gauge the potential impact of an exploited vulnerability on interconnected systems, the scope sub-factor is essential; altering the scope entails the vulnerability's capacity to influence not just the examined system, but also other systems interconnected with this AI-ML-enabled platform. This expansion can lead to an escalation of the cumulative risk. Finally, the exploit code maturity sub-factor within exploitability assesses the availability of functional exploit code. Higher risk is associated with the presence of such code, whereas minimal risk is attributed to cases where no exploit code is available, referred to as "unproven." 
% \par The concluding element within our proposed framework is the Affected User factor, designed to approximate the quantity of users impacted in the event of a vulnerability exposure. This factor operates on the principle that an increased number of affected users correlates with higher associated risk.

% \par With the essential risk analysis factors in hand for assessing AI/ML-enabled medical devices, next we furnish comprehensive descriptions for each factor to ensure consistency. {\color{black} In the previous section, we highlighted that the descriptions provided for the factors shared between our model, CVSS and DREAD are general in nature and may not be directly applicable in the healthcare context. This is a result of the varying risk levels associated with different domains, exemplified by the different risk levels when it comes to the loss of confidentiality in healthcare compared to web applications, as discussed earlier.} Detailed descriptions specific to this context can be located in the upcoming tables. Moreover, it is worth noting that when a vulnerability is exploited, the initial analysis should prioritize assessing the potential damage and exploitability. It is advisable for any analysis to adhere to this sequence before considering other factors - Affected Users, Detectability, and Ease of Mitigation - in subsequent steps. Finally, Table \ref{tab:factors} summerizes the considered factors in our proposed model.

% \begin{table*}[t]
% \centering
% \begin{tabular}{|c|M{14cm}|}
% \hline
% \textbf{Factor} & \multicolumn{1}{c|}{\textbf{Intended Use}} \\ \hline
% Damage Potential       & To assess the level of damage in case of confidentiality, integrity and availability. \\ \hline
% Exploitability        & To address how the vulnerability was exploited with several sub-factors on attack's vector and complexity, the required previliges, the need for user's interaction, the change of scope and the availability of exploit code. \\ \hline
% Affected Users        & To assess how the number of affected users by the exploited vulnerability will pose different levels of risk.
%  \\ \hline
%  Detectability        & To assess how the associated risk of an exploited vulnerability will be different based on how easy it will be detected.
%  \\ \hline
%  Ease of Mitigation        & To address if there's an available solution and who would be responsible for mitigation in case of a vulnerability being exploited.
%  \\ \hline
% \end{tabular}
% \caption{The proposed factors for risk analysis of AI/ML-enabled connected healthcare systems}
% \label{tab:factors}
% \end{table*}

% % \begin{table*}[t]
% % \centering
% % \begin{tabular}{|p{0.5in}|p{6in}|}
% % \hline
% % Risk Level & \multicolumn{1}{c|}{Descriptions} \\ \hline
% % High       & There is a complete breach of confidentiality, leading to the exposure of all resources within the affected AI/ML system to the attacker. Alternatively, the attacker may gain access to certain restricted information, but the revealed data has a direct and significant impact. For instance, the attacker could acquire the administrator's password or the private encryption keys of a web server, resulting in serious consequences.\\ \hline
% % Low        & There is a partial compromise of confidentiality. The attacker manages to gain access to certain restricted information; however, they lack control over the specific data obtained, and the extent or type of loss is restricted. The disclosed information does not result in a direct and significant loss to the affected AI/ML system.\\ \hline
% % None       & There is no loss of confidentiality within the impacted AI/ML system. \\ \hline
% % \end{tabular}
% % \caption{Confidentiality}
% % \end{table*}

% % \begin{table*}[t]
% % \centering
% % \begin{tabular}{|p{0.5in}|p{6in}|}
% % \hline
% % Risk Level & \multicolumn{1}{c|}{Descriptions} \\ \hline
% % High       & There is a complete compromise of integrity or a total breakdown of protection within the AI/ML system. For instance, the attacker gains the ability to modify any or all files safeguarded by the system. Alternatively, although only certain files can be modified, any malicious alterations would result in direct and significant consequences for the affected system.
% % \\ \hline
% % Low        & It is possible to modify the data within the AI/ML system; however, the attacker lacks control over the consequences of the modifications, or the extent of modification is restricted. The data alterations do not result in a direct and significant impact on the affected system.
% % \\ \hline
% % None       & There is no loss of integrity within the impacted AI/ML system. \\ \hline
% % \end{tabular}
% % \caption{Integrity}
% % \end{table*}

% % \begin{table*}[t]
% % \centering
% % \begin{tabular}{|p{0.5in}|p{6in}|}
% % \hline
% % Risk Level & \multicolumn{1}{c|}{Descriptions} \\ \hline
% % High       & There is a complete loss of availability within the AI/ML system, enabling the attacker to fully deny access to its resources. This loss of availability can either be sustained, meaning the attacker continues to deliver the attack, or persistent, where the condition persists even after the attack has concluded. Alternatively, the attacker possesses the capability to partially disrupt availability, but this loss of availability has a direct and serious impact on the affected system. For example, the attacker may be unable to disrupt existing connections but can prevent new connections, or they can repeatedly exploit a vulnerability that, although each successful attack only leaks a small amount of memory, eventually leads to a complete unavailability of the service.
% % \\ \hline
% % Low        & The performance of the AI/ML system is diminished, or there are intermittent disruptions in the availability of its resources. Even if the vulnerability can be repeatedly exploited, the attacker lacks the capability to entirely block access for legitimate users. The resources within the affected system are either partially available consistently or fully available intermittently. However, overall, there is no immediate and significant impact directly affecting the affected system.
% % \\ \hline
% % None       & There is no impact to availability within the impacted AI/ML system. \\ \hline
% % \end{tabular}
% % \caption{Availability}
% % \end{table*}

% \begin{table*}[t]
% \centering
% \begin{tabular}{|c|c|M{14cm}|}
% \hline
% Sub-factor & Risk Level & \multicolumn{1}{c|}{Description}                                         \\ \hline
% & High & There is a complete breach of confidentiality, leading to the exposure of all resources within the affected AI/ML system to the attacker. Alternatively, the attacker may gain access to certain restricted information, but the revealed data has a direct and significant impact. For instance, the attacker could acquire the administrator's password or the private encryption keys of a web server, resulting in serious consequences. \\ \cline{2-3} 
% & Low & There is a partial compromise of confidentiality. The attacker manages to gain access to certain restricted information; however, they lack control over the specific data obtained, and the extent or type of loss is restricted. The disclosed information does not result in a direct and significant loss to the affected AI/ML system. \\ \cline{2-3} 
% \multirow{-8}{*}{\begin{sideways} Confidentiality \end{sideways}} & None & There is no loss of confidentiality within the impacted AI/ML system.         \\ \hline
% & High & There is a complete compromise of integrity or a total breakdown of protection within the AI/ML system. For instance, the attacker gains the ability to modify any or all files safeguarded by the system. Alternatively, although only certain files can be modified, any malicious alterations would result in direct and significant consequences for the affected system. \\ \cline{2-3} 
% & Low & It is possible to modify the data within the AI/ML system; however, the attacker lacks control over the consequences of the modifications, or the extent of modification is restricted. The data alterations do not result in a direct and significant impact on the affected system.                                                   \\ \cline{2-3} 
% \multirow{-5}{*}{\begin{sideways} Integrity \end{sideways}} & None & There is no loss of integrity within the impacted AI/ML system.                         \\ \hline
% & High  & There is a complete loss of availability within the AI/ML system, enabling the attacker to fully deny access to its resources. This loss of availability can either be sustained, meaning the attacker continues to deliver the attack, or persistent, where the condition persists even after the attack has concluded. Alternatively, the attacker possesses the capability to partially disrupt availability, but this loss of availability has a direct and serious impact on the affected system. For example, the attacker may be unable to disrupt existing connections but can prevent new connections, or they can repeatedly exploit a vulnerability that, although each successful attack only leaks a small amount of memory, eventually leads to a complete unavailability of the service. \\ \cline{2-3} 
%  & Low  & The performance of the AI/ML system is diminished, or there are intermittent disruptions in the availability of its resources. Even if the vulnerability can be repeatedly exploited, the attacker lacks the capability to entirely block access for legitimate users. The resources within the affected system are either partially available consistently or fully available intermittently. However, overall, there is no immediate and significant impact directly affecting the affected system.                                        \\ \cline{2-3} 
% \multirow{-12}{*}{\begin{sideways} Availability \end{sideways}}    & None & There is no impact to availability within the impacted AI/ML system.            \\ \hline
% \end{tabular}
% \caption{Damage Potential}
% \end{table*}

% % \begin{table*}[t]
% % \centering
% % \begin{tabular}{|p{0.5in}|p{6in}|}
% % \hline
% % Type & \multicolumn{1}{c|}{Descriptions} \\ \hline
% % Network       & The AI/ML system is susceptible to remote attacks originating from the internet. This type of vulnerability, referred to as 'remotely exploitable,' enables targeting the system from a distance, potentially spanning multiple routers.
% % \\ \hline
% % Adjacent        & The AI/ML system is network-connected, but the attack is constrained to a specific level within the network structure. This limitation implies that the attack can only occur from a logically adjacent area, which may include the same physical or logical network, such as Bluetooth or a local IP subnet. Additionally, the attack could originate from within a secure or restricted administrative domain, such as MPLS or a secure VPN connecting to an administrative network zone.
% % \\ \hline
% % Local       & The AI/ML system is not directly connected to the network, and the attacker can exploit the vulnerability either locally (e.g., keyboard, console), or remotely (e.g., SSH). \\ \hline
% % Physical & The attack in this case necessitates the physical interaction with the AI/ML system which can be a brief interaction (e.g., an evil maid attack).
% % \\ \hline
% % \end{tabular}
% % \caption{Attack Vector}
% % \end{table*}

% % \begin{table*}[t]
% % \centering
% % \begin{tabular}{|p{0.5in}|p{6in}|}
% % \hline
% % Risk Level & \multicolumn{1}{c|}{Descriptions} \\ \hline
% % High       & For a successful attack to occur, certain conditions must be met that are beyond the control of the attacker. This means that the attacker cannot simply launch the attack whenever they want. Instead, they must invest a significant amount of effort in preparation or execution against the AI/ML system before they can expect the attack to be successful. 
% % \\ \hline
% % Low        & There are no special access conditions or exceptional circumstances required for the attack. An attacker can expect a successful attack when targeting the AI/ML system.\\ \hline
% % \end{tabular}
% % \caption{Attack Complexity}
% % \end{table*}

% % \begin{table*}[t]
% % \centering
% % \begin{tabular}{|p{0.5in}|p{6in}|}
% % \hline
% % Risk Level & \multicolumn{1}{c|}{Descriptions} \\ \hline
% % High       & The attacker requires privileges that grant substantial control (e.g., administrative privileges) over the AI/ML system, enabling access to its settings and files.\\ \hline
% % Low        & The attacker requires privileges that grant basic user capabilities, typically limited to modifying settings and files owned by a user. Alternatively, an attacker with low privileges has the ability to access only non-sensitive resources.\\ \hline
% % None       & The attacker, being unauthorized prior to the attack, does not necessitate any access to settings or files of the AI/ML system in order to execute an attack. \\ \hline
% % \end{tabular}
% % \caption{Privileges Required}
% % \end{table*}

% % \begin{table*}[t]
% % \centering
% % \begin{tabular}{|p{0.5in}|p{6in}|}
% % \hline
% % Type & \multicolumn{1}{c|}{Descriptions} \\ \hline
% % Required       & For successful exploitation of the vulnerability, a user needs to perform a specific action before the vulnerability can be exploited. For instance, a successful exploit may only occur during the installation of an application by a system administrator.\\ \hline
% % None       & The vulnerable AI/ML system can be exploited without requiring any user interaction. \\ \hline
% % \end{tabular}
% % \caption{User Interaction}
% % \end{table*}

% % \begin{table*}[t]
% % \centering
% % \begin{tabular}{|p{0.5in}|p{6in}|}
% % \hline
% % Type & \multicolumn{1}{c|}{Descriptions} \\ \hline
% % Changed       & An exploited vulnerability can have an impact on resources that extend beyond the security scope managed by the security authority of the vulnerable AI/ML system. In this scenario, the vulnerable system and the affected components are distinct and managed by different security authorities.\\ \hline
% % Unchanged        & An exploited vulnerability can exclusively impact resources that fall under the management of the same security authority. In this scenario, the vulnerable AI/ML system and the affected components are either identical or both are under the management of the same security authority. \\ \hline
% % \end{tabular}
% % \caption{Scope}
% % \end{table*}

% % \begin{table*}[t]
% % \centering
% % \begin{tabular}{|p{0.5in}|p{6in}|}
% % \hline
% % Type & \multicolumn{1}{c|}{Descriptions} \\ \hline
% % High       & There is functional autonomous code available, or in some cases, no exploit is required as the vulnerability can be triggered manually. Comprehensive details regarding the vulnerability are widely accessible. The exploit code is effective in every situation, or it is actively being disseminated through an autonomous agent such as a worm or virus.\\ \hline
% % Functional        & There is available functional exploit code that effectively operates in various scenarios where the vulnerability is present. The code demonstrates its efficacy across a wide range of situations where the vulnerability is exploitable.\\ \hline
% % Proof-of-Concept       & Proof-of-concept exploit code is accessible, or in some cases, an attack demonstration may not be feasible for most systems. However, it is important to note that the provided code or technique may not be fully functional in all situations and could necessitate significant modifications by a skilled attacker.
% %  \\ \hline
% % Unproven & No exploit code is available, or an exploit is theoretical. \\ \hline
% % \end{tabular}
% % \caption{Exploit Code Maturity}
% % \end{table*}

% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage[table,xcdraw]{xcolor}
% % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[t]
% \begin{tabular}{|c|c|M{13.5cm}|}
% \hline
% Sub-factor & Type/Risk Level & \multicolumn{1}{c|}{Description} \\ \hline
% & Network & The AI/ML system is susceptible to remote attacks originating from the internet. This type of vulnerability, referred to as 'remotely exploitable,' enables targeting the system from a distance, potentially spanning multiple routers. \\ \cline{2-3} 
% & Adjacent & The AI/ML system is network-connected, but the attack is constrained to a specific level within the network structure. This limitation implies that the attack can only occur from a logically adjacent area, which may include the same physical or logical network, such as Bluetooth or a local IP subnet. Additionally, the attack could originate from within a secure or restricted administrative domain, such as MPLS or a secure VPN connecting to an administrative network zone.                            \\ \cline{2-3} 
% & Local  & The AI/ML system is not directly connected to the network, and the attacker can exploit the vulnerability either locally (e.g., keyboard, console), or remotely (e.g., SSH).                               \\ \cline{2-3} 
% \multirow{-9}{*}{\begin{sideways} Attack Vector \end{sideways}} & Physical  & The attack in this case necessitates the physical interaction with the AI/ML system which can be a brief interaction (e.g., an evil maid attack).           \\ \hline & High            & For a successful attack to occur, certain conditions must be met that are beyond the control of the attacker. This means that the attacker cannot simply launch the attack whenever they want. Instead, they must invest a significant amount of effort in preparation or execution against the AI/ML system before they can expect the attack to be successful.                                        \\ \cline{2-3} 
% \multirow{-4}{*}{\begin{sideways} \begin{tabular}[c]{@{}c@{}}Attack \\ Complexity\end{tabular} \end{sideways}} & Low           & There are no special access conditions or exceptional circumstances required for the attack. An attacker can expect a successful attack when targeting the AI/ML system.                                      \\ \hline & High & The attacker requires privileges that grant substantial control (e.g., administrative privileges) over the AI/ML system, enabling access to its settings and files.                                       \\ \cline{2-3} 
% & Low & The attacker requires privileges that grant basic user capabilities, typically limited to modifying settings and files owned by a user. Alternatively, an attacker with low privileges has the ability to access only non-sensitive resources. \\ \cline{2-3} 
% \multirow{-4}{*}{\begin{sideways} \begin{tabular}[c]{@{}c@{}}Privileges \\ Required\end{tabular} \end{sideways}}   & None & The attacker, being unauthorized prior to the attack, does not necessitate any access to settings or files of the AI/ML system in order to execute an attack. \\ \hline
% & Required  & For successful exploitation of the vulnerability, a user needs to perform a specific action before the vulnerability can be exploited. For instance, a successful exploit may only occur during the installation of an application by a system administrator.  \\ \cline{2-3} 
% \multirow{-4}{*}{\begin{sideways} \begin{tabular}[c]{@{}c@{}}User \\ Interaction\end{tabular} \end{sideways}}      & None & The vulnerable AI/ML system can be exploited without requiring any user interaction. \\ \hline & Changed & An exploited vulnerability can have an impact on resources that extend beyond the security scope managed by the security authority of the vulnerable AI/ML system. In this scenario, the vulnerable system and the affected components are distinct and managed by different security authorities. \\ \cline{2-3} 
% \multirow{-4}{*}{\begin{sideways} Scope \end{sideways}}                 & Unchanged & An exploited vulnerability can exclusively impact resources that fall under the management of the same security authority. In this scenario, the vulnerable AI/ML system and the affected components are either identical or both are under the management of the same security authority.  \\ \hline & High & There is functional autonomous code available, or in some cases, no exploit is required as the vulnerability can be triggered manually. Comprehensive details regarding the vulnerability are widely accessible. The exploit code is effective in every situation, or it is actively being disseminated through an autonomous agent such as a worm or virus. \\ \cline{2-3} 
% & Functional  & There is available functional exploit code that effectively operates in various scenarios where the vulnerability is present. The code demonstrates its efficacy across a wide range of situations where the vulnerability is exploitable.  \\ \cline{2-3} 
% & Proof-of-Concept & Proof-of-concept exploit code is accessible, or in some cases, an attack demonstration may not be feasible for most systems. However, it is important to note that the provided code or technique may not be fully functional in all situations and could necessitate significant modifications by a skilled attacker.  \\ \cline{2-3} 
% \multirow{-9}{*}{\begin{sideways} Exploit Code Maturity \end{sideways}} & Unproven   & No exploit code is available, or an exploit is theoretical.  \\ \hline
% \end{tabular}
% \caption{Exploitability}
% \end{table*}

% \begin{table*}[t]
% \centering
% \begin{tabular}{|c|M{14cm}|}
% \hline
% Type & \multicolumn{1}{c|}{Descriptions} \\ \hline
% All Users       & The vulnerability in the AI/ML system affects all users which can lead to significant consequences for everyone involved. \\ \hline
% Some Users        & The vulnerability in the AI/ML system has an impact on select users, targeting specific subsets within the user base and resulting in limited consequences for that particular portion. \\ \hline
% Single User       & The vulnerability in the AI/ML system is targeted or localized, typically affecting a single individual or a small number of people.
%  \\ \hline
% \end{tabular}
% \caption{Affected User}
% \end{table*}

% \begin{table*}[t]
% \centering
% \begin{tabular}{|c|M{14cm}|}
% \hline
% Risk Level & \multicolumn{1}{c|}{Descriptions} \\ \hline
% High       & It is unlikely to easily find the vulnerability in the AI/ML system and it requires a remarkable amount of time and effort. \\ \hline
% Medium        & Detecting the potential for malicious exploitation in this vulnerability in the AI/ML system requires thoughtful consideration and analysis, as it operates at a level that may not be immediately apparent. \\ \hline
% Low       & The vulnerability in the AI/ML system can be easily identified through a few basic observations, posing minimal challenge in its detection. \\ \hline
% \end{tabular}
% \caption{Detectability}
% \end{table*}

% % \begin{table*}[t]
% % \centering
% % \begin{tabular}{|p{0.5in}|p{6in}|}
% % \hline
% % Type & \multicolumn{1}{c|}{Descriptions} \\ \hline
% % Security Researcher       & The main responsibility of the security researchers lies in responsibly disclosing vulnerabilities and ensuring the information reaches the appropriate entity. The risk in this process can be the potential miscommunication, delay in reporting, or incomplete understanding of the vulnerability in the AI/ML system in comparison to other responsible entities, which could hinder the mitigation process. \\ \hline
% % Third-party Vendor        & If the vulnerability within the AI/ML system can be exploited using any of its components, it becomes the responsibility of the third-party vendor, acting as the manufacturer, to either enhance the design of the component or replace it with a more reliable alternative. \\ \hline
% % Technology Vendor       & Failure to promptly release patches or updates to fix vulnerabilities can leave users exposed to potential attacks. With the complete knowledge about the design of the AI/ML system, vendors must thoroughly investigate reported vulnerabilities, develop effective patches to ensure proper mitigation. \\ \hline
% % System Administrator & If administrators – as the frontline entity to deal with the vulnerabilities - fail to promptly apply patches or implement necessary security measures, the risk of successful attacks targeting the vulnerabilities increases. Therefore, their actions directly impact the mitigation of the vulnerabilities in the AI/ML system they manage. \\ \hline
% % \end{tabular}
% % \caption{Responsible Entity}
% % \end{table*}

% % \begin{table*}[t]
% % \centering
% % \begin{tabular}{|p{0.5in}|p{6in}|}
% % \hline
% % Type & \multicolumn{1}{c|}{Descriptions} \\ \hline
% % Unavailable      & Either a feasible solution does not exist or, if one does, it proves impossible to implement. \\ \hline
% % Workaround     & An unofficial, non-vendor solution exists, where users or administrators of AI/ML may take matters into their own hands by creating a patch or providing steps to mitigate the vulnerability. In certain cases, individuals within the user community offer alternative measures or workarounds to address or minimize the impact of the vulnerability. \\ \hline
% % Temporary Fix       & An official but temporary solution is available, which may include the vendor providing a temporary hotfix, tool, or workaround. In such cases, the vendor acknowledges the issue and offers a temporary measure to address the vulnerability until a permanent fix can be developed and implemented. \\ \hline
% % Official Fix & A comprehensive vendor solution is available, either in the form of an official patch released by the vendor or through an available upgrade. This means that the vendor has provided a complete resolution to address the vulnerability, offering users or administrators the means to apply an official fix or update to mitigate the risk effectively. \\ \hline
% % \end{tabular}
% % \caption{Responsible Entity}
% % \end{table*}

% \begin{table*}[t]
% \begin{tabular}{|c|c|M{13.5cm}|}
% \hline
% Sub-factor & Type & \multicolumn{1}{c|}{Description} \\ \hline & \begin{tabular}[c]{@{}c@{}}Security \\ Researcher\end{tabular} & The main responsibility of the security researchers lies in responsibly disclosing vulnerabilities and ensuring the information reaches the appropriate entity. The risk in this process can be the potential miscommunication, delay in reporting, or incomplete understanding of the vulnerability in the AI/ML system in comparison to other responsible entities, which could hinder the mitigation process.         \\ \cline{2-3} 
% & \begin{tabular}[c]{@{}c@{}}Third-party\\ Vendor\end{tabular}   & If the vulnerability within the AI/ML system can be exploited using any of its components, it becomes the responsibility of the third-party vendor, acting as the manufacturer, to either enhance the design of the component or replace it with a more reliable alternative.     \\ \cline{2-3} 
% & \begin{tabular}[c]{@{}c@{}}Technology\\ Vendor\end{tabular}    & Failure to promptly release patches or updates to fix vulnerabilities can leave users exposed to potential attacks. With the complete knowledge about the design of the AI/ML system, vendors must thoroughly investigate reported vulnerabilities, develop effective patches to ensure proper mitigation.            \\ \cline{2-3} 
% \multirow{-11}{*}{\begin{sideways} Responsible Entity \end{sideways}} & \begin{tabular}[c]{@{}c@{}}System\\ Administrator\end{tabular} & If administrators – as the frontline entity to deal with the vulnerabilities - fail to promptly apply patches or implement necessary security measures, the risk of successful attacks targeting the vulnerabilities increases. Therefore, their actions directly impact the mitigation of the vulnerabilities in the AI/ML system they manage.         \\ \hline
% & Unavailable & Either a feasible solution does not exist or, if one does, it proves impossible to implement. \\ \cline{2-3} 
% & Workaround & An unofficial, non-vendor solution exists, where users or administrators of AI/ML may take matters into their own hands by creating a patch or providing steps to mitigate the vulnerability. In certain cases, individuals within the user community offer alternative measures or workarounds to address or minimize the impact of the vulnerability.  \\ \cline{2-3} 
% & \begin{tabular}[c]{@{}c@{}}Temporary\\ Fix\end{tabular} & An official but temporary solution is available, which may include the vendor providing a temporary hotfix, tool, or workaround. In such cases, the vendor acknowledges the issue and offers a temporary measure to address the vulnerability until a permanent fix can be developed and implemented.                                                      \\ \cline{2-3} 
% \multirow{-7.5}{*}{\begin{sideways} Remediation Level \end{sideways}}  & Official Fix & A comprehensive vendor solution is available, either in the form of an official patch released by the vendor or through an available upgrade. This means that the vendor has provided a complete resolution to address the vulnerability, offering users or administrators the means to apply an official fix or update to mitigate the risk effectively. \\ \hline
% \end{tabular}
% \caption{Ease of Mitigation}
% \end{table*}


% % \begin{itemize}
% %     \item a table containing the factors and sub-factors?
% %     %\item An opening paragraph to recall why it is important to have a risk analysis: 
% %     %\item Start with Detection and Responsible Entity and make examples in BGMS
% %     %\item continue with other factors and mention how the descriptions are justified with respect to the context
% % \end{itemize}

% %\par TBD: Table to show assessment of the risks identified in Section \ref{sec:attacks} according to the proposed framework.

==> sections/future-directions.tex <==
\section{Future Research Directions}\label{sec:future}
Amidst the growing trend in the adoption of ML-enabled medical systems and personalized treatment plans, it becomes imperative to ensure the security of these medical systems. The insights that we obtained from analyzing the state-of-the-art risk assessment techniques and commercial ML-enabled medical systems open up the following interesting interdisciplinary research directions.


\noindent\textbf{Automated risk identification.} While early identification and mitigation of security risks in ML-enabled medical systems is necessary, it is highly challenging owing to the multi-vendor nature of the systems and their compatibility with a wide range of peripheral devices. In this work, we identified the risks by manually going through several online resources (device descriptions, research articles, and vulnerability databases). However, such manual analysis is neither practical nor scalable to industry standards. Therefore, automating the risk identification and analysis process would benefit device manufacturers as well as the security research community. This is not a trivial task, as this would require identifying relevant documents on the web and parsing a huge volume of unstructured documents, while at the same time being able to relate various ML concepts in a relevant manner. Therefore, designing an automated risk identification technique would possibly require novel natural language processing techniques, and could be an interesting research direction.

\noindent\textbf{A new risk assessment framework for ML-enabled medical systems. }In Section \ref{sec:existingframeworks} we showed that state-of-the-art risk assessment techniques are not sufficient for assessing the severity of the security risks in ML-enabled connected medical systems. Accurate assessment of such risks would require translating the risk severity in peripheral devices to the risk severity of the overall system, and thereby, the impact on a targeted patient. Developing such a risk assessment technique would require interdisciplinary knowledge, especially in the domains of system security and medicine. The risk assessment technique should also provide guidance to security practitioners about which risks to prioritize and which manufacturer to hold responsible for mitigating a given risk. This too is a multi-faceted problem that would require analyzing the time, effort and expenses required to mitigate a given risk and its impact on the vulnerable patients. Hence, we need a new risk assessment framework for assessing the risks in ML-enabled connected medical systems.

\noindent\textbf{Building personalized spatial and temporal risk profiles per patient.} 
% The results of our case study show that some patients are more vulnerable than others to our proposed attack.
The results of our case study show that when an ML-enabled medical system is attacked, the mispredictions cause more damage to certain patients than they cause to others. At the same time, a patient is not equally vulnerable throughout the day, i.e., they might be more vulnerable at different times of the day (for example, before having food as opposed to after having food). An interesting research problem is to study patients' data in more detail to develop customized spatial and temporal risk profiles for every patient which would allow us to better understand why some patients are more vulnerable than others, and at what points in time are they most vulnerable. The insights from this analysis would help security researchers develop efficient risk mitigation strategies.

\noindent\textbf{Designing efficient risk mitigation techniques.} Designing an efficient risk mitigation technique in this domain is a necessary yet challenging task, and involves addressing the following research problems.
    \begin{enumerate}
        \item \textbf{Building robust and attack-resilient ML models.} As we have seen in our case study, the impact of cyber-attacks on ML models have different impact on different patients. Once a patient's spatial and temporal risk profile is known, researchers can understand with greater certainty the circumstances under which the patient is likely to be the worst affected in the face of an attack. This would then help security researchers develop universal attack strategies that would perform equally well on all the patients regardless of their risk profiles. In the security research domain, developing strong attack techniques is important for evaluating the resilience of systems against strong adversaries. Therefore, once a powerful universal attack is devised, researchers should invest time and resources into developing a robust and resilient defense technique that would cater to the discrepancies in the spatial and temporal risk profiles of individual patients.
        \item \textbf{Enforcing accountability in risk mitigation strategy.} \gargi{This can be removed in case of a space crunch. I have mentioned this as a problem under 'new risk assessment framework...'} In any multi-vendor system, deciding which manufacturer should be held accountable for mitigating risk is not straightforward for security auditors. Especially in safety-critical infrastructures such as medical systems, the security auditor should put the responsibility on the party who can mitigate the risk at the earliest, and in a way that is convenient to the patients. For instance, in the case of our BGMS attack, building and installing a patch for the ML-enabled software would be more beneficial for patients than waiting for the Bluetooth protocol developers to fix the root cause of the vulnerability. Also, sometimes a company is reluctant to fix an issue because they do not have enough financial incentive to do so. Even when a company takes up the responsibility of risk mitigation, the first solution might not be the best one. 
        It should also be noted that sometimes implementing temporary and substandard solutions (e.g., keeping a vulnerable system disconnected from the Internet) is necessary as that might be the best immediate solution to a problem. However, the auditor must ensure that the responsible manufacturer is making steady progress toward developing the most effective solution as early as possible. Enforcing such accountability in the domain of ML-enabled medical systems might require revisiting and redefining cybersecurity policies with the best interest of patients in mind. 
    \end{enumerate}

    
    
    % \item \textbf{Build ML models that are more robust and resilient to adversarial attacks.} Once a patient's personalized spatial and temporal profile is known, researchers and developers can now understand with greater certainty the points at which the patient is at their weakest level in the face of an attack. This would then help researchers and practitioners develop stronger adversarial attacks that are more universal in nature, meaning that the attack could perform equally well on all the patients regardless of their risk profiles. However, the development should not stop at this point. Instead, once a powerful universal attack that exploits the vulnerabilities of individual patients is devised, researchers and practitioners should invest time and resources into developing a robust and resilient defense technique that would cater to the discrepancies in the spatial and temporal risk profiles of individual patients.


==> sections/introduction_bkp_0.tex <==
\section{Introduction}\label{sec:intro}

The use of Artificial Intelligence (AI), especially Machine Learning (ML) techniques, is becoming increasingly popular in medical fields in recent years. As of October 2022, the U.S. Food and Drug Administration (FDA) has approved $521$ ML-enabled devices across $15$ different medical disciplines (e.g., Cardiology, Ophthalmology, and Gastroenterology)~\cite{fdaml}. These medical devices are used for performing critical activities such as remote patient monitoring~\cite{rx1}, controlling surgical equipment~\cite{7d}, automatic drug administration~\cite{dreamed}, and preliminary/advanced disease diagnosis~\cite{cardiologs} -- tasks that require predicting the patients' medical conditions with high accuracy, reliability, and availability. Wrong predictions made by ML techniques can have a wide range of catastrophic consequences, such as wrong treatment leading to health complications, and even death. Therefore, there is a compelling need to protect ML-enabled medical systems from cyberattacks. 

Existing research works~\cite{pitropakis2019taxonomy,chen2020ecgadv,albattah2023detection,chen2019shapeshifter,lal2021adversarial,9313421,joel2021adversarial,bortsova2021adversarial,menon2021covid,vargas2020understanding,levy2022personalized,chen2022adversarial,yu2023perturbing,nielsen2022investigating,mangaokar2020jekyll,hu2022adversarial,ma2021understanding} 
% \karthik{Why are there no citations in the introduction? This is strange!}
across various application areas have shown that ML engines are vulnerable to cyber-attacks. An adversary can force an ML engine to produce incorrect predictions or decisions by injecting carefully crafted adversarial data points either during training or inference. To prevent and mitigate these attacks, regulatory organizations such as the FDA recommend addressing cybersecurity concerns during the design and development of medical systems~\cite{fdapremarket}. For this, a thorough risk~\footnote{In this paper, risk is the probability of a security vulnerability getting exploited, and its potential impact or loss~\cite{risk}.} analysis of these systems is necessary to identify, prioritize, and systematically mitigate potential security risks. 

Performing a risk assessment of ML-enabled medical devices during its early stages of development is challenging. An ML-enabled device, such as one approved by the FDA, is only a decision-making component of a much larger connected medical system. At deployment, this ML-enabled device is interfaced with several other peripheral devices, each of which may be manufactured by a different company. For instance, a user of the ML-enabled diabetes management app Dreamed Advisor Pro~\cite{dreamed}, needs to install the app on a smartphone, and then connect to it a smartwatch, a glucose meter, and an insulin pump, all of which can be manufactured by different other companies, and have their own security vulnerabilities. Even if the app developer ensures that the ML engine is secure, adversaries can still exploit vulnerabilities in the peripheral devices and communication channels to inject adversarial data points into the ML engine. Furthermore, each app user may use peripheral devices from different sets of manufacturers, leading to diverse vulnerabilities among different users of the same app. It is challenging for the app developer to estimate how the different vulnerabilities would enable an adversary to achieve a specific goal.
 % Today, it is challenging for the manufacturer to identify these risks in the early stages of development. 

\IEEEpubidadjcol

% In this paper, we first show some real-world instances, where even if the ML-enabled device (hardware/software) is secure, an adversary can inject malicious data points into the ML engine by exploiting vulnerabilities in the connected peripheral devices. 
% % \karthik{Where are these studies?}\gargi{Here I meant the studies we performed in Section-3. Should we add a reference here?} %It is unlikely for medical practitioners to know which of the connected devices might have security vulnerabilities, and 
% % It is unlikely for the ML engine designer to know which peripheral devices the customers would connect to the ML engine at deployment, and which of them may have security vulnerabilities. It is also challenging to estimate how the different vulnerabilities would enable an adversary to craft and inject adversarial data points into the ML engine to achieve a specific goal.
% % Such risks are difficult to identify during the product design phase without a complete view of the end-to-end system. 
% To the best of our knowledge, today there is no systematic methodology for 
% % \karthik{Rephrased this as framework is not necessary for risk assesment}
% %no state-of-the-art framework that helps 
% manufacturers and security practitioners to perform a comprehensive end-to-end risk analysis (identification and severity assessment) of medical systems. While individual medical devices are sometimes tested in silos, no risk analysis is performed on the end-to-end system. Moreover, the in-silo assessments only account for conventional enterprise attacks or software vulnerabilities.
% % Moreover, the ML-enabled devices approved by FDA have been tested only for accuracy and security against conventional enterprise attacks, and not for their trustworthiness under adversarial scenarios. 
% This leaves potential security risks due to vulnerabilities in peripheral devices undetected. 

In this paper, we show real-world scenarios where an adversary can compromise the security of an ML-enabled device by injecting malicious data through connected peripheral devices, even when the ML-enabled device itself is secure. Currently, there is no systematic method for manufacturers and security experts to conduct a comprehensive end-to-end risk identification and severity assessment in ML-enabled connected medical systems. Presently, individual medical devices are tested in isolation and these isolated assessments typically focus only on traditional enterprise attacks and software vulnerabilities, overlooking potential security risks arising from vulnerabilities in peripheral devices.

The high-level objective of this work is to build a framework for systematically identifying and assessing the severity of security risks in AI/ML-enabled connected medical systems during the product design and development phase. 
While early identification of security risks is important for early risk mitigation, severity assessment is important for determining the risks that should be prioritized for mitigation and for designing efficient risk mitigation strategies. 

Designing the risk analysis framework consists of three steps. \textit{First}, we conduct a systematic exploration of the FDA-approved ML-enabled medical devices to understand the ML techniques that they use and the damages that can be caused to a patient if the ML technique mispredicts their case. \textit{Second}, we conduct an extensive literature review to \textit{identify} possible ways in which adversaries can inject malicious data points into an ML-enabled medical device at deployment. This involves a cross-domain analysis, where we map known attacks on ML algorithms with known vulnerabilities in peripheral devices that would make the attacks practical. \textit{Next}, we perform a critical evaluation of state-of-the-art risk assessment frameworks used by the ML-enabled medical device manufacturing companies today. We identify loopholes in these risk assessment strategies that might make manufacturers miss the risks arising due to vulnerabilities in connected peripheral devices. \textit{Finally}, based on the insights obtained from the aforementioned analyses, we design a risk \textit{assessment} technique that considers the impact of the identified risks on the end-to-end system, and thereby, the patient. 


% The risk assessment technique qualitatively assesses the identified risks according to the following five parameters - \textit{(1) Damage potential -} This indicates the nature of the damage caused to the patients (loss of privacy, integrity, or confidentiality); \textit{(2) Exploitability -} This indicates the ease of executing the attack. This depends on factors such as whether the attack can be executed remotely, reproduced on similar medical systems at different instances of time, the technical expertise required by an adversary, and the cost of exploitation; \textit{(3) Affected users -} This is an estimate of the number of patients who would be affected if the vulnerability is exploited; \textit{(4) Detectability -} This indicates how easy it would be to identify the vulnerability for the attack; and, \textit{(5) Ease of mitigation -} This indicates the ease with which a risk can be 
% % \karthik{We should define risk somewhere.} 
% mitigated, once identified. These parameters have been used to design the framework to conform to the guidelines issued by the National Institute of Standards and Technology (NIST) for ensuring the trustworthiness of AI/ML-enabled systems~\cite{tabassi2023artificial}. While the parameters themselves are not new, the novelty of this work is mapping the risks to these parameters, while considering \textit{(i)} how different combinations of vulnerabilities in the peripheral devices put the ML engine at risk, and \textit{(ii)} how practical it is for an adversary to exploit those vulnerabilities. 

Finally, we present a case study to demonstrate how the proposed end-to-end risk analysis framework would help security auditors and device manufacturers identify and mitigate security risks in a realistic AI/ML-enabled medical system, namely, a blood glucose monitoring system (BGMS). First, we demonstrate a practical attack on the BGMS to show how an attacker can exploit the vulnerabilities in connected peripheral devices to make the ML engine prescribe fatal doses of insulin to the patient. We follow up by showing how our risk analysis framework would have identified and helped mitigate the risk in the early stages of the design and development of this system.


% of applying the risk assessment framework in an AI/ML-enabled diabetes management system.
% \karthik{We need to say more about what this case study does, and what we demonstrate with it. }

% This SoK is primarily intended for security auditors and manufacturers of AI/ML-enabled medical devices. 
The risk identification method proposed in this paper would help the device manufacturers foresee risks that might arise at the time of deployment. Early identification of risks can help manufacturers incorporate appropriate attack mitigation mechanisms in their design. This would save them the time, money, and effort that they would incur in designing patches or recalling their products if the risks were identified after deployment. The risk analysis method proposed in this paper would help security auditors develop standard guidelines for enforcing accountability in the event of a security breach in multi-vendor ML-enabled medical systems.
% \karthik{What about other researchers?}
Insights obtained from this work can also aid regulatory bodies in designing new guidelines and regulations to enforce risk analysis in ML-enabled medical devices. Finally, we also present some insights regarding the mitigation of the risks identified, which will help security researchers pave the way for the development of secure and trustworthy medical systems.
% \ldots \textbf{TBD: Points on how they will benefit from this work}

\noindent\textbf{Contributions. }The main contributions of this paper are as follows.
\begin{enumerate}
    \item We perform a systematic cross-domain security analysis of commercial ML-enabled medical devices (Section \ref{sec:attacks}) and a critical evaluation of state-of-the-art risk assessment techniques (Section \ref{sec:existingframeworks}) to show that current risk assessment techniques are inadequate in identifying and analyzing the severity of security risks in ML-enabled medical systems. Specifically, the state-of-the-art techniques fail to identify risks posed to the ML engine by vulnerable peripheral devices.
    \item Based on the insights obtained from the study above, we propose a new risk assessment technique that identifies and analyzes the severity of security risks not only on the ML-enabled device but also on the end-to-end ML-enabled medical system (Section \ref{sec:framework}). The proposed technique would help in the identification and mitigation of security risks in the early stages of device development, and would therefore reduce the health risks of patients and the financial risks of the manufacturers.
    \item We demonstrate the effectiveness of the proposed risk assessment technique by performing a case study on a realistic ML-enabled blood glucose monitoring system (Section \ref{sec:case-study}). For this, we first demonstrate an attack on the system where we assume that the adversary can compromise a Bluetooth communication link in the system. Next, we show how the proposed risk analysis technique would have averted such an attack.
    \item Finally, we present a discussion on potential research directions identified from this work (Section \ref{sec:future}).
\end{enumerate}





